MicroGlam: Microscopic Skin Image Dataset with Cosmetics

In this paper, we present a cosmetic-specific skin image dataset. It consists of skin images from $45$ patches ($5$ skin patches each from $9$ participants) of size $8mm^*8mm$ under three cosmetic products (i.e., foundation, blusher, and highlighter). We designed a novel capturing device inspired by Light Stage. Using the device, we captured over $600$ images of each skin patch under diverse lighting conditions in $30$ seconds. We repeated the process for the same skin patch under three cosmetic products. Finally, we demonstrate the viability of the dataset with an image-to-image translation-based pipeline for cosmetic rendering and compared our data-driven approach to an existing cosmetic rendering method.

==> acknowledgment.tex <==
\section{Acknowledgment}
We thank all subjects who participated in the capture sessions. This work is supported in part by Value Exchange Engineering, a joint research project between R4D, Mercari Inc. and the RIISE, JSPS Grant-in-Aid JP23K16921, JST AdCORP JPMJKB2302, and by NSF OISE 2153560.


==> conf_preamble.tex <==
\RequirePackage{ifthen}
\newcommand{\conf}{siggraph}
% submit, camera, final....
\newcommand{\stage}{final}
% \newcommand{\track}{journal}
% \def\conf{cvpr}
% \input{siggraph_preamble}
\newcommand{\isequal}[3]{
    \ifthenelse{\equal{#1}{#2}}{
        #3
    }{}    
}

\isequal{\conf}{siggraph}{\input{siggraph/siggraph_preamble}}
\isequal{\conf}{cvpr}{\input{cvpr/cvpr_preamble}}
\isequal{\conf}{eccv}{\input{eccv/eccv_preamble}}
\isequal{\conf}{uist}{\input{uist/uist_preamble}}
\isequal{\conf}{chi}{\input{chi/chi_preamble}}
\isequal{\conf}{pg}{\input{cgf/cgf_preamble}}
\isequal{\conf}{tvcg}{\input{ieeetrans/ieeetrans_preamble}}

% \ifthenelse{\equal{\conf}{siggraph}}{
%     \input{siggraph/siggraph_preamble}
% }
% {
% }

% \ifthenelse{\equal{\conf}{cvpr}}{
%     \input{cvpr/cvpr_preamble}
% }
% {
% }

% \ifthenelse{\equal{\conf}{eccv}}{
%     \input{eccv/eccv_preamble}
% }
% {
% }

% \ifthenelse{\equal{\conf}{uist}}{
%     \input{uist/uist_preamble}
% }
% {
% }

==> overview.tex <==
\section{Overview}
